Perceiving Physical Equation by Observing Visual Scenarios

Inferring universal laws of the environment is an important ability of human intelligence as well as a symbol of general AI. In this paper, we take a step toward this goal such that we introduce a new challenging problem of inferring invariant physical equation from visual scenarios. For instance, teaching a machine to automatically derive the gravitational acceleration formula by watching a free-falling object. To tackle this challenge, we present a novel pipeline comprised of an Observer Engine and a Physicist Engine by respectively imitating the actions of an observer and a physicist in the real world. Generally, the Observer Engine watches the visual scenarios and then extracting the physical properties of objects. The Physicist Engine analyses these data and then summarizing the inherent laws of object dynamics. Specifically, the learned laws are expressed by mathematical equations such that they are more interpretable than the results given by common probabilistic models. Experiments on synthetic videos have shown that our pipeline is able to discover physical equations on various physical worlds with different visual appearances.

==> nips_2018 arxiv/qual_fig.tex <==

\begin{figure}

\centering

\begin{tabular}{c}
\toprule[1pt]\midrule

\subfigure{
\begin{minipage}[c]{0.4\linewidth}
\centerline{\textbf{Physical Scenario}}
\end{minipage}
\begin{minipage}[c]{0.28\linewidth}
\centerline{\textbf{Learned} $\Delta d_x$}
\end{minipage}
\begin{minipage}[c]{0.28\linewidth}
\centerline{\textbf{Learned} $\Delta d_y$}
\end{minipage}
}

\\\midrule

%drift
\subfigure{
\begin{minipage}[c]{0.4\linewidth}
\centering
\includegraphics[width=0.32\linewidth]{700010000.jpg}
\includegraphics[width=0.32\linewidth]{700010050.jpg}
\includegraphics[width=0.32\linewidth]{700010099.jpg}
\centerline{\textbf{Dirft}~(\url{http://bit.ly/2L6JR8W})}
\end{minipage}
\begin{minipage}[c]{0.28\linewidth}
\centering
\includegraphics[scale=0.6]{tree_drift_1.png}
\small
\begin{equation}
v_x \Delta t \notag
\end{equation}
\end{minipage}
\begin{minipage}[c]{0.28\linewidth}
\centering
\includegraphics[scale=0.6]{tree_drift_2.png}
\small
\begin{equation}
v_y \Delta t  \notag
\end{equation}
\end{minipage}
}

\\\midrule

%apple
\subfigure{
\begin{minipage}[c]{0.4\linewidth}
\centering
\includegraphics[width=0.32\linewidth]{500070000.jpg}
\includegraphics[width=0.32\linewidth]{500070050.jpg}
\includegraphics[width=0.32\linewidth]{500070099.jpg}
\centerline{\textbf{Free-falling}~(\url{http://bit.ly/2k3HIyu})}
\end{minipage}
\begin{minipage}[c]{0.28\linewidth}
\centering
\includegraphics[scale=0.7]{tree_0.png}
\small
\begin{equation}
0 \notag
\end{equation}
\end{minipage}
\begin{minipage}[c]{0.28\linewidth}
\centering
\includegraphics[scale=0.55]{tree_apple_2.png}
\small
\begin{equation}
v_y \Delta t - 4.907\Delta t^2 \notag
\end{equation}
\end{minipage}
}

\\\midrule

%parabola
\begin{minipage}[c]{0.4\linewidth}
\centering
\includegraphics[width=0.32\linewidth]{400010000.jpg}
\includegraphics[width=0.32\linewidth]{400010050.jpg}
\includegraphics[width=0.32\linewidth]{400010099.jpg}
\centerline{\textbf{Parabola}~(\url{http://bit.ly/2It4Kcq})}
\end{minipage}
\begin{minipage}[c]{0.28\linewidth}
\centering
\includegraphics[scale=0.6]{tree_parabola_1.png}
\small
\begin{equation}
v_x \Delta t \notag \notag
\end{equation}
\end{minipage}
\begin{minipage}[c]{0.28\linewidth}
\centering
\includegraphics[scale=0.55]{tree_parabola_2.png}
\small
\begin{equation}
v_y \Delta t - 4.888\Delta t^2 \notag
\end{equation}
\end{minipage}

\\\midrule

%slope
\subfigure{
\begin{minipage}[c]{0.4\linewidth}
\centering
\includegraphics[width=0.32\linewidth]{300030000.jpg}
\includegraphics[width=0.32\linewidth]{300030055.jpg}
\includegraphics[width=0.32\linewidth]{300030099.jpg}
\centerline{\textbf{Slope}~(\url{http://bit.ly/2L7CIF1})}
\end{minipage}
\begin{minipage}[c]{0.28\linewidth}
\centering
\includegraphics[scale=0.55]{tree_slope_1.png}
\small
\begin{equation}
v_x \Delta t + 4.920\sin \theta \cos \theta \Delta t^2 \notag
\end{equation}
\end{minipage}
\begin{minipage}[c]{0.28\linewidth}
\centering
\includegraphics[scale=0.55]{tree_slope_2.png}
\small
\begin{equation}
v_y \Delta t - 4.911\sin ^2 \theta \Delta t^2 \notag
\end{equation}
\end{minipage}
}

\\\midrule

\subfigure{
\begin{minipage}[c]{0.4\linewidth}
\centering
\includegraphics[width=0.32\linewidth]{200000000.jpg}
\includegraphics[width=0.32\linewidth]{200000041.jpg}
\includegraphics[width=0.32\linewidth]{200000099.jpg}
\centerline{\textbf{Spring}~(\url{http://bit.ly/2KuAfnj})}
\end{minipage}
\begin{minipage}[c]{0.28\linewidth}
\centering
\includegraphics[scale=0.7]{tree_0.png}
\small
\begin{equation}
0 \notag
\end{equation}
\end{minipage}
\begin{minipage}[c]{0.28\linewidth}
\centering
\includegraphics[scale=0.5]{tree_spring_2.png}
\small
\begin{equation}
v_y \Delta t - (d_y+10019.555) /m \cdot \Delta t^2 \notag
\end{equation}
\end{minipage}
}

\\ \midrule \bottomrule[1pt]
\end{tabular}

\caption{\textbf{Physical scenarios and our learned equations.} In each scenario, the object moves under particular dynamic equations. Please click the URLs to watch the synthetic videos if interested. Results show that our method is able to learn correct mathematical equations with relatively accurate physical constants in all of the scenarios. The syntax trees are shown together with the equations. The images are resized to 600$\times$600 for visual clarity.}
\label{qualitative_fig}
\end{figure}
